PRSNet: Part Relation and Selection Network for Bone Age Assessment

Bone age is one of the most important indicators for assessing bone's maturity, which can help to interpret human's growth development level and potential progress. In the clinical practice, bone age assessment (BAA) of X-ray images requires the joint consideration of the appearance and location information of hand bones. These kinds of information can be effectively captured by the relation of different anatomical parts of hand bone. Recently developed methods differ mostly in how they model the part relation and choose useful parts for BAA. However, these methods neglect the mining of relationship among different parts, which can help to improve the assessment accuracy. In this paper, we propose a novel part relation module, which accurately discovers the underlying concurrency of parts by using multi-scale context information of deep learning feature representation. Furthermore, based on the part relation, we explore a new part selection module, which comprehensively measures the importance of parts and select the top ranking parts for assisting BAA. We jointly train our part relation and selection modules in an end-to-end way, achieving state-of-the-art performance on the public RSNA 2017 Pediatric Bone Age benchmark dataset and outperforming other competitive methods by a significant margin.

==> method.tex <==
\section{Method}
\label{sec:method}

%\di{I have to say this overview is really, really poor. It does not give any information. Check our ECCV or CVPR paper, and rewrite it...} In this paper, we propose the Part Relation and Selection Network for bone age assessment, more specifically, the PRSNet consists of 2 modules, a part relation module and a part selection module, as illustrated in Fig. \ref{overall}.
%In order to build strong relation between the parts in X-ray images, we adopt the part relation modules into the backbone to generate the global feature with rich contextual information, moreover, these modules provide feature as part selection module's input. The details will be described in section 2.2.
%Next, the part selection module will use the features provided by part relation module to implement the anchor scoring. According to the score, we select the most useful parts in images as local network's input, hence the discriminative local feature will be learned, we will described more details in section 2.3.
%Moreover, the gender information is kind of important prior knowledge for bone age assessment, we use the fully connection convolution to exact gender feature. Final, the global, local feature as soon as the gender feature will cooperate for joint learning and prediction, the concept will be elaborated in Section 2.4.



\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth,height=0.3\linewidth]{figures/overview.pdf}
\caption{.}
\vspace{-0.1in}
\label{fig:overview}
\end{figure*}

\subsection{Part Relation Module}

The task of bone age assessment  based on the synthetic consideration of parts in hands, hence building a strong part relation throughout X-ray images is the initial stage yet crucial stage, only the correct and necessary connections were made in various parts of hand,the model can make sensitive and precise prediction. 
However, recently works use only single part of images as input , which neglects parts' relation, leads to limited performance. To address this problem, some works further extract feature on whole image directly to yield richer information, however the large variation of bone with respect to positions, sizes, shapes causes model to product amount of negative evidence, making they yield a poor and chaotic part relation.

In this paper, we propose the Part Relation Module to build a strong and fine relationship between the parts, the details are demonstrated in Fig. \ref{part_relation}. The module aims to suppress activation in the irrelevant regions and highlight response in informative regions, which make the connection between parts more directly and observably, the rich context information among parts can be embedded into the local representation. We apply the part relation module into serval level feature in the network, enabling the model to handle the part relation in different scales and embed the contextual information from coarse to fine(hierarchy).
 
Frist, the module generates a relation map, which identifies salient image regions and prune feature responses to preserve only the activations relevant to the bone. Then, we implement element-wise multiplication of the relation map and trunk feature to attain the gating vetor, which contain the contextual information. Finally, we sum the residual feature and the gating feature, embedding the context information between parts into the flow feature. The part relation module can be formulated as follows:

\begin{figure}[ht]
	\centering
	\includegraphics[width=1\textwidth]{figures/Attention/part_relation.pdf}
	\vspace{+0.5em}
	\caption{Schematic of the proposed Part Relation Module, }
	\label{part_relation}
\end{figure}

\begin{equation} \label{eq1}
\widehat{X} = ((W^T_tX_i + b_t) \cdot \sigma(W^T_cX_i + b_c)) + (W^T_rX_i + b_r)
\end{equation}
where the $\sigma() = \frac{1}{1+exp(-(W^T_cX_i + b_c))}$   corresponds to the sigmoid activation function, the Part Relation Module is characterised by a set of parameters $\theta_r$ containing: linear transformations $W_c\in \mathbb{R}^{F_c \times F_{int}} $,$W_t\in \mathbb{R}^{F_t \times F_{int}} $,$W_r\in \mathbb{R}^{F_r \times F_{int}} $ and the bias terms $b_c, b_t, b_r \in \mathbb{R}$, in here, the linear transformations are computed using channel-wise 1x1x1 convolutions for the input tensor, which is referred to as vector concatenation-based attention. We would like to note the part relation module can be inserted into any architecture easily with a few extra parameters and can be optimized by standard back-propagation.

\subsection{Part Selection Module}

%part 和 patch 应该如何对应起来
In clinical bone age diagnosis, the radiologists will give more attention to some anatomic parts , which are more representative and discriminative. And recent methods use single fixed part of images as prior input, even model can learn discriminative representations more easily, it's performance is limited due to neglect parts relation, moreover, these methods select parts fixedly and need expensive preprocessing. In this paper, we adovate that the primise of good part relation, selecting the most useful parts for futher study can benefit model's learning of discriminative feature, and hence boost the performance.

To achieve this goal, we propose the part selection module to select the most informative parts for further study. Based on the self-supervision mechanism, our model can search and select parts without any human annotations.

Inspired by the idea of proposals based on anchors in object detection, we use the anchors mechanism to constitute a proposals set:$A = \left\{A_1, A_2, ...A_n \right\}$, which denotes the list of possible important part.  Relying on setting of sizes and ratios, the anchor can locate any possible parts in variou sizes, the detail of anchor setting is illustrated in Fig. \ref{anchor}.  Correspondingly, we will implement the anchor scoring, which uses the features provided by the Part Relation Modules to regress the score for each anchor. As a result, we can attain the anchor scores : $S = \left\{S_1, S_2, ...S_n \right\}$, and the $S_n$ represents the informativeness of the anchor $A_n$.
Then, we will perform the selection step, selecting most important part for further study. Frist, we sort the anchor list:$A$ and implement the non maximum suppression to avoid excessive overlap, then we will pick out the top-$M$ anchors and crop patches in original image by corresponding coordinates of anchors. And these patches will be fed into a local network:VGG-16 to exact more discriminative local feature.
However, the operation of cropping is differentiable, which causes the Part Selection Module unable to update parameters via standard gradient backpropagation.
To address this problem, we adopt the ranking loss in work\cite{yang2018learning}, which enable the Part Selection Module to be optimized by standard backpropagation. The ranking loss mainly consist of 2 parts:the information function and confidence function, the information function  $I:A \rightarrow (-\infty, +\infty) $ is defined to evaluate how informative the parts are, and in here, we use the mean square loss function as the $I$, and then confidence function $C:A \rightarrow [0, 1] $ is setted as a classifier to evaluate the confidence of part's representativeness, we use the anchor scoring to denote this function. With the assumption that the more informative and useful part should have higher confidence, so the following condition should hold:

\begin{equation} \label{eq2}
\left\{(A_i, A_j),C(A_i) > C(A_j) \lvert I(A_i)>I(A_j)\right\}
\end{equation}

we denote the Top-$M$ parts as $\left\{P_1, P_2, ...P_m \right\}$, each parts will be resize to a uniform size and generate predict results via the local network. Then their informativeness will be produced by the mean square loss, which represent as $I$ =  $\left\{I_1, I_2, ...I_m \right\}$. Therefore, the ranking loss is defined as follow:
\begin{equation} \label{eq3}
L_{rank}(I,C) = \sum_{(i,j):C_i<C_j} f(I_j - I_i)
\end{equation}

Similar to the work\cite{yang2018learning}, we use the hinge loss function  $f(x) = max\left\{1-x, 0\right\}$ to stimulate  $I_i > I_j$ if the $C_i > C_j$, therefore, the Part Selection Module can pickout the most useful parts in X-ray image for further study, and the more discriminative local feature provided by the Part Selection Module will joint the global feature and gender feature to make more sensitive, precise prediction, the parameters in Part Selection Module can be optimized by normal gradient backpropagation.
\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.037]{figures/Attention/anchor_setting.pdf}
	\vspace{+0.5em}
	\caption{Illustration of the anchor setting in the part selection module. Totally, we set the three sizes of anchors with three ratios}
	\label{anchor}
\end{figure}

\subsection{Network Training}
The part relation module and part selection module are the relationship of mutual promotion, mutual reliance, whicih jointly distill data feature for BAA, moreover, due to the gender information is also important in BAA, we exact the gender feature to assist training and prediction. We concatenate the global feature, local feature and gender feature to regress a joint logit, which represenets the final prediction, and there are three not independent but rather complementary losses for our proposed PRSNet. Hence, the total optimization loss function is defined as:
\begin{equation} \label{eq3}
L_{total} = L_{joint} + \alpha*L_{full} + \beta*L_{rank}
\end{equation}
where the $L_{full}$ and $L_{joint}$ represent the mean square loss function for full logit and joint logit. and the  $L_{rank}$ denotes the ranking loss, which's input include the confidence and informative of picked parts, and we set the loss weight: $\alpha$ and $\beta$ as 1,1.



